Collaborative Job Seeking for People with Autism: Challenges and Design Opportunities

Successful job search results from job seekers' well-shaped social communication. While well-known differences in communication exist between people with autism and neurotypicals, little is known about how people with autism collaborate with their social surroundings to strive in the job market. To better understand the practices and challenges of collaborative job seeking for people with autism, we interviewed 20 participants including applicants with autism, their social surroundings, and career experts. Through the interviews, we identified social challenges that people with autism face during their job seeking; the social support they leverage to be successful; and the technological limitations that hinder their collaboration. We designed four probes that represent major collaborative features found from the interviews--executive planning, communication, stage-wise preparation, and neurodivergent community formation--and discussed their potential usefulness and impact through three focus groups. We provide implications regarding how our findings can enhance collaborative job seeking experiences for people with autism through new designs.

==> subsections/04_S1result.tex <==
\section{Study 1: Findings}

We provide the perspectives of our three main stakeholders structured in four themes: (1) Challenges in Job Seeking, (2) Drivers in Job Seeking, (3) Autism Characteristics in Job Seeking, and (4) Awareness between and beyond the Stakeholders.
The first theme explores the Seekers' challenges during their career search along with their coping strategies and support from their networks.
The second theme explores the drivers in job search, including building a network, leveraging external connections, identifying useful features in existing tools, and conducting pre-assessments to better characterize the individual profile and their strengths. 
The third theme illustrates challenges faced by people with autism, drawing from prior work.
Lastly, our final theme discusses how awareness can be raised between and beyond the stakeholder groups.
\subsection{\textbf{Challenges in Job Seeking}}

In this section, we present the challenges that people with autism face in their job search. We focus on (1) Searching and Applying for jobs, (2) Preparing the Application Materials, and (3) Proceeding with Interviews.
We share perspectives from our stakeholders and explore how Seekers, Surroundings, and Experts work collaboratively to manage these challenges through coping strategies. 


Standard strategies for searching and applying for jobs used by neurotypical job seekers may not be effective for individuals on the autism spectrum.
Also, the lack of guidance and knowledge about the process prevents them from effectively leveraging relevant resources and connections.
Seekers recognize the importance of networking while looking for job opportunities, however, they are unsure about how to do it effectively.
As P5 illustrates, \textit{``I had reached out to various professors to ask if they knew of anything because everybody tells you it's all about connections and stuff. But that wasn't very fruitful either''}.
Engaging in interpersonal interactions within the same workgroup and collecting information is often a straightforward process for neurotypicals, however, people with autism often encounter challenges with it.

Some participants expressed a lack of confidence or doubts in their skills, which deterred them from applying for a job. 
As P18 mentioned, \textit{``I think the only challenge we've really had is me not wanting to apply for a job because I don't believe I'm qualified''}.
Searching based on individual criteria and preferences~\cite{annabi_locke_2019} poses a challenge and limits the pool of suitable options.
Specifically, wanting work accommodations, including remote work, no relocation requirements, or a large company, limits the job options.
As P6 mentioned, \textit{``If it's reachable by public transportation, I could move there. But right now, I prefer to be 100\% remote''}.
Preference is also related to the type of work, as P16 said, \textit{``One of the challenges with my profile is that I am not particularly good at a lot of entry-level work. I am better in a kind of mid-level experience or senior-level position where you deal more with concepts''}
Participants expressed their frustrations with existing job search platforms as they produce overwhelming results with irrelevant information. 

\textbf{(b) Coping Strategies:}
Establishing connections with current employees and references are valuable for job seekers to can gain insights about the company and available positions.
As P1 mentioned: \textit{``I ended up talking to one of my friends who was working in a biomedical engineering lab. She walked me through what she did to get into that lab, I followed her advice and it worked, I got into that lab''}.
P16 mentioned that a direct reference from his friend helped his application bypass the computer-based filtering system and get called.
Defining specific job requirements prevents confusion and increases interest among the applicants. 
As P5 mentioned,\textit{``I was glad about that they weren't looking for someone with years of experience. It was kind of interesting because everyone was really inclined to hire''}. 
Searching for jobs based on given criteria and being selective to match personal interest is effective.

Career coaches and expert professionals provide valuable information and resources to support seekers.
P10 explained how she connects them to recruiters, \textit{``I will check in with them more regularly, or actually make the connection with the recruiter for them over email. I'll give them resources for them to find''}.
P13 emphasizes that multiple resources are recommended to collect information, \textit{``We use multiple platforms and websites because comprehensive information isn't available in a single location.''}.
Career coaches also compile information regarding accommodation needs for each job seeker, facilitating a more inclusive and accessible job search.
As P19 mentioned, \textit{``I support placing them in a position that is the right position for them. So what we want to avoid is a job placement that's not appropriate for that individual, whether that's because their skill set is not lined up well, whether the location''}.
The level of support and engagement from experts varies based on individual needs.

\subsubsection{\textbf{Preparing Application Materials}}

\paragraph{}

\textbf{(a) Challenges:}
Seekers expressed frustration when preparing application documents, including resumes, cover letters, and emails.
P1 mentioned challenges to structuring her resume and writing emails, \textit{``I've been trying to structure my resume so that it's easy for recruiters to read, but I haven't been able to find any information on how to do that .... Communication through email is always difficult for me because I hate writing emails to begin with, and I am not great at introducing myself''}.
Seekers also struggle to determine the level of detail in writing emails, for example, P4 said, \textit{``Sometimes when I'm going over stuff in so much detail, it will exhaust the people I'm talking to''}.
Keeping track of the applications, organizing and consolidating the information from scattered resources is difficult, as P4 said, \textit{`` everything is so scattered is the part of the problem, you have to go to many different tools and make sure you're getting that together and organized somewhere so that all are enlisted''}. 


Seekers shared their frustration due to the inadequacy of feedback and updates about applications despite investing significant effort.
As P5 said, \textit{``I had been applying to jobs I saw on LinkedIn, but so many times I never heard back. I sent follow-up emails, I never got responses. It was so disheartening and frustrating.''}.
Candidates typically require feedback about their application to move forward in their search.
The prolonged uncertainty increases their anxiety and leads to disappointment.
As P1 said, \textit{``It's like if I'm just spouting out into the world and not getting any feedback''}.
P17 from the Surroundings group highlighted the challenge of dealing with unclear timelines and delays in receiving feedback from employers, \textit{``It's a very frustrating experience. When he applied for this job, the lack of communication and the absence of a straightforward process were evident. They didn't give us any timelines or information''}.


\paragraph{}

\textbf{(b) Coping Strategies:}
Seekers benefit from feedback on their applications, including verifications,  proofreading, help with interview preparation, and resume building~\cite{annabi_locke_2019, Lashkari_2023}.
The most common and effective strategy adopted was involving family members and Surroundings in the process~\cite{10.1145/3476065}.
For example, P1 shared, \textit{``I had my parents look over my resume, and they gave me feedback on it. We've gone through quite a few iterations. My dad works in IT, so he understands at least the technical aspects of things. My mom's pretty good at people skills, she helped out how to word things so that they sound confident''}.



Experts are involved in preparing, and monitoring the progress of job applications and provide feedback to ensure the Seeker's needs are met and their applications are progressing.
As P19 shared, \textit{``We'll also do resume development if that's required, as well as interview preparation. So we do a lot of interview preparation to lessen the anxiety that takes place there''}.
P10 said she follows up with individuals with autism more frequently, \textit{``For the neurodiverse population I follow up about how the application's been going. I have more frequent appointments with them, and I also have more frequent email communication''}.
Organizing the tasks and work materials in personalized ways is also helpful in increasing the Seeker's task efficiency and productivity.
Specifically, P8 prefers paper planners rather than calendar apps, \textit{``I use a paper planner that breaks down my day into 30-minute increments so I can easily see the amount of time I need to dedicate to tasks that are not related to the job search process''}.



\subsubsection{\textbf{Proceed with the Interviews}}

\paragraph{}

\textbf{(a) Challenges:}
Current job interviews are challenging for Seekers as they often require memorization and quick thinking, which do not always align with the strengths and needs of individuals with autism.
As P4 remarked, \textit{``I think the typical process is fairly problematic because it's a lot of on-the-fly stuff in your head that you have to just memorize stuff''}.
A candidate's capacity to memorize and recall answers during an interview does not always accurately reflect their talent or suitability for a position.
Also, it creates additional pressure on the Seekers as they strive to maintain a positive image during the interviews.
For instance, P6 mentioned \textit{``Sometimes, they throw out a question unexpectedly that might not be possible for me to answer immediately. I had to keep in mind that I would have to look positive based on my appearance''}.
People with autism often rely on prepared scripts to navigate interviews, and when confronted with questions out of their scripts, they face challenges in forming appropriate responses spontaneously.

A misalignment between the applied job and the candidate's personal interests causes stress, as P5 stated, \textit{``I'm very passionate about my work and I think I would feel more nervous for an interview if I was not interested in the work I was doing''}.
Misunderstanding and missing the context is another issue that Seekers face and it hinders getting proper information during interviews. 
As P1 said, \textit{``A lot of times, I miss the mark. It kind of derails the process of actually making that connection and getting the information that both of us need. Especially in interviews, the interviewer is looking for something, and I don't know what they're looking for. I have an idea of what I'm looking for''}.

\paragraph{}

\textbf{(b) Coping Strategies:}
Offering guidance for interview preparation, by sharing questions in advance, providing follow-up sessions after the interview for Seekers to modify their responses, or allowing more time during the interview is beneficial.
As P4 said, \textit{``I don't like to think of all the things during the meeting. Getting the questions in advance can be very helpful. Or having a follow-up in two hours, I'll have 10 other ideas of useful information I could give you''}.
Career coaches provide support to arrange informational interviews between recruiters and job seekers to gain insights about a company's culture and discover job opportunities.
For instance, P10 said, \textit{``I still encourage them to do it because it's really the fantastic way to learn what you want to do based on people's real-life experiences and build your network when you're applying to jobs''}.


Scripting is found to be useful and the right length of script provides Seekers with structured guidance to better navigate during the interview.
P20 mentioned while creating scripts anticipating the questions beforehand was helpful for her,\textit{``For every interview I often prepped like 6 to 10 pages of a script. Basically, I used my experiences as a PM and also research to figure out what likely questions people are going to ask''}.
Our participants also mentioned the usefulness of the counter script that provides alternative explanations for potential concerns raised during the interview. 
For instance, if someone is late to the interview, a counter script could explain it as a situation where they initially arrived on time but had to return for forgotten keys, etc.
As per the recommendations of Experts, job seekers can adopt a proactive approach by requesting the accommodations they need before attending an interview.
Instead of explicitly discussing their autism, explaining how these accommodations will enable them to perform at their best can be a good strategy.



\subsection{\textbf{Drivers in Job Seeking}}

This section introduces Drivers, which are influential factors that positively reinforce the job search process for people with autism.

\subsubsection{\textbf{Connecting to People with Autism}}

12 participants emphasized the value of connecting with other neurodivergent individuals since it is easier for them to relate to and share experiences with people who may have similar traits.
As P1 said, \textit{``So maybe it's just I click with other neurodiverse people''}.
P16 also talked about connecting with an entrepreneur who has a similar profile to him.
They shared the same understanding and communication was easy, as P16 mentioned,\textit{``We had an amazing conversation. I felt a great connection with it. Because we have a similar profile. We both lack a bunch of social skills. We can talk about socioeconomic, politics, and science and be on a similar level''}.
Expert group participant P13 mentioned the importance for the neurodiverse community to find others who can relate to their experiences and with whom they can ``unmask'', or be their authentic selves, \textit{``I always want people to find other neurodivergent people who get them, with whom they can unmask. I always want to support people in finding others who understand them''}.

Building connections with other individuals on the autism spectrum who have successfully secured jobs can provide valuable insights for seekers as well as tips.
For example, P6 mentioned, \textit{``it is better to make more connections with people who are like neurodiverse candidates and who were able to get a job. To know what tips they have, or what employers to look for''}.
This provides a sense of community and belonging, as Seekers can relate to shared challenges and experiences in the job market and also gain confidence that meaningful employment is achievable.
However, people with autism may not naturally initiate social interactions because it may not be their preference.
P9 from the Surroundings group discussed this issue and suggests that external motivation or facilitation is needed to make this happen, \textit{``I do think that it can be helpful, as long as it is being initiated by an outside person. Because what happens with people on the spectrum is they don't initiate very well on their own. The group would have to be motivated to show up and initiate a conversation between themselves, for it to be effective''}.


\subsubsection{\textbf{Connecting to External Network}}

Our stakeholders recognized that connecting with outside networks is beneficial for job seeking.  
P1 talked about the scopes of networking and mentorship in academia, as professors often connect students with opportunities and resources in their field of study.
Career fairs and events are great opportunities for networking and discovering job openings. 
Same for P4 as well, \textit{``My first job was right out of college and that, I got through a job fair I believe at the at the university''}.
Seekers utilize social media and job sites to collect information about opportunities and contact personnel. 

Maintaining relationships and leveraging connections with professionals and career development support play a significant role in achieving one's goals~\cite{annabi_locke_2019}.
As P16 said, \textit{``I guess I prepared myself by getting a degree by working with an occupational therapist (OT) to try and set myself up for meetings and all kinds of other things like that''}.
P6 mentioned that these connections are valuable to receive support and updated opportunities, \textit{``I frequently contact the connections I made at school and with CAI. Anything I need, they help me out. They also help me keep up connections, keep me notified, and stay up-to-date with whatever is going on or any advice I might need''}.
Even after a rejection, maintaining contact with companies to understand their needs is beneficial (P11).

\subsubsection{\textbf{Existing Job Seeking Platform Features}}

Our participants expressed mixed feelings and challenges while using widely known job searching platforms such as, LinkedIn, Indeed, Monster.com~\cite{linkedin, indeed, mosnter, ziprecruiter}.
The \textbf{most disliked features of these tools include search criteria, filtering options, matched results or outcomes, complex navigation, and social media-like attributes}.
Here are some statements of their feelings regarding these tools:
P5: \textit{``I found Linkedin and those sorts of things exhausting. It's really hard to find things on them. You search for a term, and like 80 things that are relevant come up''}.
P6: \textit{``On LinkedIn It's very unclear. What a free-level position requirements are like, It's even harder to find. A good job from a company that's accepting of neurodiverse, candidates like myself''}.
P8: \textit{``That Linkedin has struck me as like a professional version of Facebook. It seems to be more socially oriented, and a geared towards growing connections. I have tried ZipRecruiter, monster.com. Indeed seems to be, the most comprehensive as well in terms of the amount of positions that are advertised on the site''}.
P14: \textit{``I'm very discouraging in general of people just applying through Indeed, because I think it's a black hole''}.
P9:\textit{``You really don't know what you're getting in Indeed, it's vague. You're just doing what's usually a quick application''}.
P14 raised concerns about ONET by the Department of Labor resources~\cite{ONET}, that this system is designed for a broad audience and the suggestions are not suitable for Seekers.

These examples emphasize the importance of considering alternative job search strategies and platforms.
Our participants shared their experiences of using resources that are designed and tailored specifically for neurodivergent individuals.
For instance, Mentra~\cite{WinNT3} is a hiring platform that intelligently searches and matches job for neurodivergent individuals~\cite{WinNT3}. 
P5 found it useful as the Seekers are guided through questions during the account creation to identify the support or accommodations they require. 
P14 liked the feature that Mentra creates an opportunity for organizations and groups that focus on recruiting neurodivergent individuals, \textit{``Mentra is one potential there are some good groups out there who are specifically recruiting their divergent individuals and there they sign on with employers''}.
P16 talked about another tool MindShift~\cite{mindshift} that offers support of job coaching and human resources expertise to understand accommodation needs for an individual. 
He identified a limitation of this tool that it limits their support to job opportunities within only the companies that are in contract with them. 
If an individual is interested in a job at a company that is not part of MindShift's contracts, they may not receive the assistance.
P15 mentioned a management tool SetWorks~\cite{serworks} that their company uses.
The tool contains comprehensive participant profiles and a historical record of interactions with employers from past employees, which is vital information for current job hunters.
By allowing them to review past employer feedback about specific companies, it assists them in making more informed decisions. 


\subsubsection{\textbf{Pre-Assessments and Identifying the Needs}}

Conducting pre-assessments at the beginning of a job search is  important, serving as a foundational step to customize job search strategies and employment opportunities to align with the Seeker's unique needs and strengths.
For instance, neuropsychological assessments provide valuable insights into an individual's cognitive and behavioral functioning, helping to identify strengths and weaknesses.
P11 emphasized how a comprehensive assessment is influential to understand an individual's unique profile that can be shared with employers, \textit{``Neuropsychological assessment is so crucial because when they reach adulthood point, there's hardly any support out there for these kids. I would say if you have a child who has more severe symptoms and attributes of this profile then you need that assessment. Because that assessment then could be looked at with an employer''}.
P14 mentions her approaches to helping a Seeker which begins with a functional assessment, where they consider various aspects of the individual's life outside of work, such as their living situation and overall well-being.
Sometimes Seekers may overestimate their abilities and claim they can do more than they are realistically capable of. 
This can ultimately be detrimental to the individual's success.
To address this issue, P15 emphasizes the importance of conducting assessments to accurately identify a Seeker's capabilities and limitations
Along with the same line of thought, P19 pointed out the significance of the initial intake process when working with Seekers.
In this step, collecting information about the individual's background, experiences, and aspirations helps them to understand their challenges and needs.
Involving Surroundings in the process is also strategic because the collaborative approach provides comprehensive support to Seekers.

\subsection{\textbf{Autism Characteristics in Job Seeking}}
In this section, we emphasize the barriers that stem from the inherent characteristics of autistic job seekers, which are also confirmed in past literature. 

\subsubsection{\textbf{Executive Planning}}

Our participants talked about executive functioning challenges~\cite{LUNA2007474, liss_fein_allen, Van} related to managing multiple tasks, problem-solving, switching between tasks, and effectively organizing resources that are cognitively demanding for the seekers.
For example, P16 mentioned, \textit{``Where I found more difficulties was working with the Department of Vocational Rehabilitation was they wanted me to apply for 10 different jobs every week. That's a lot of paperwork and a lot of task-switching that I'm not good at. That's gonna be very expensive for my energy levels''}.
Engaging in thinking on the spot is cognitively demanding and not preferable, as P4 said, \textit{``Like in a meeting, I don't think of all the things during the meeting''}.
Some participants had difficulties in maintaining the necessary level of attention, especially while checking email inboxes, notifications, etc. which can result in missing important information.
The constant need to be vigilant for upcoming schedules, tracking carefully, and timely responding can introduce fatigue issues.
P4 shared how alarm fatigue can divert someone from doing the actual task, \textit{``There can be so many alarms going off all the time that the one that warns about what somebody should be doing right now, does not capture their attention. So false alarms are very problematic''}.

\subsubsection{\textbf{Social Communication}}

The Seekers shared their experiences of having social anxiety and communication~\cite{rubin2004challenges, biklen1990communication, picard2009future} issues including initiating conversation, mixing with other people, and difficulties in reading or understanding social cues and signals during their career search. 
P1 felt stressed while attending a mandatory post-interview social gathering at a bar, \textit{``Straight after all the interviews they go to a bar and they're like, 'Okay, now socialize.' It's supposed to be like a de-stress sort of thing, but socializing is not really de-stressing for me''}.
Being a team player, assisting, and providing support to other people is another inherent challenge that Seekers face.
Some participants blamed the lack of emotional intelligence and social skills as blockers to their personal growth in fighting social awkwardness.

Another common barrier our participants addressed is the issue of communication between neurodiverse and neurotypical individuals.
Comprehending a neurotypical behavior within a conventional social context can result in miscommunication and misunderstandings.
P20 said, \textit{``That was something very hard for me to deal with in terms of aggressive people or communication can be judgmental when it comes off that way''}.
People with autism face challenges in grasping subtleties, unspoken contexts, and hidden meanings.
Understanding the job-related subtleties and figuring out the unspoken rules is difficult for Seekers because these nuances are not explicitly communicated, which are grasped by neurotypicals naturally.
Navigating social situations is challenging for neurodiverse individuals~\cite{rubin2004challenges}, and they need extra patience and understanding while communicating with them.

\subsubsection{\textbf{Propensity of Literal Thinking}}

People with autism tend to interpret language and words in a very concrete and straightforward manner~\cite{hobson2012autism}.
P12 from the expert group who also has autism, emphasizes this issue, \textit{``We are very literal thinkers, if you say one thing with the literal definition of your words, but means something else we're very likely to get confused. For ASD-level ones with minimal difficulties, verbalizing miscommunications is probably the number one issue that we have''}.
In written communication, such as emails or documents, Seeker's perspectives are sometimes interpreted as blunt or straightforward, as P4 said, \textit{``A lot of the content is in my writing style and I also deliberately used a “critical studies” writing style which is very much different from what a lot of people see, but the Washington Post journalist described it as blunt''}.
Job advertisements often use complex language, euphemisms(P8), and extensive lists of qualifications, that make job seekers consider themselves not qualified for the position being sought.
Interview questions that can have countless potential responses are difficult to handle for the Seekers, as P16 mentioned, \textit{``There are some standard interview questions like, “Tell me about yourself” that I find incredibly challenging, you know. Tell me about yourself has almost infinite possibilities''}.

\subsubsection{\textbf{Emotional Regulation}}

Managing rejections, coping with disappointment, and handling emotions are some challenges~\cite{samson2012emotion, MAZEFSKY2013679, Samson_Hardan} that individuals with autism face during their job seeking journey.
For instance, P16 mentioned, \textit{``If I get a second or third interview, I get really excited and I start creating fantasies about what my job is going to look like and what my life is going to be like in 5 or 10 years. So then, when I don't get the job, it's really painful and very frustrating. If I'm trying to manage disappointment and setbacks, it's not so good''}.
We identified from seeker group participants that their mood and energy levels influence their capacity to effectively utilize social connections in their career search. 
As P16 stated, \textit{``if I am in a very positive, optimistic place then I think I could possibly leverage my surroundings and social connections to help get me jobs. If it doesn't work out well or something If my mood is low, energy is low, then what I project is not something that people want to help or support, or that employers would be interested in''}.
Like anyone else, people with autism seek the autonomy to make decisions by themselves and desire independence in their actions, which may not be easy to achieve. 
P11 remarked on her son's feelings, \textit{``He wants to stand on his own and he doesn't want his mother telling him how he should act and what he should say''}.
Another observation is in situations where social interactions or workplace dynamics deviate from the expected, such situations can be harder for them to process and think about, possibly due to the cumulative effect of negative feedback they receive throughout their lives.
As P11 mentioned, \textit{``Imposter syndrome or just thinking that we're not doing a good enough job, those anxieties and worries are even more pronounced for these individuals because they've had so much negative feedback their whole life''}.

\subsection{Awareness between and beyond the Stakeholders}

In this section, we explore the potential collaborative steps that should be taken by three types of stakeholders and employers to raise awareness in multiple directions to mitigate the challenges.
\paragraph{}
\textbf{From Surroundings to Seekers: } 
Recognizing the unique needs of individuals with autism is crucial for their family members, enabling them to offer essential support and advocacy. 
As P9 believes her son has all positive qualities attractive to employers, he only requires explicit direction and specific guidance to navigate and cope with the social cues that he finds challenging. 
Support from one's surroundings, as emphasized by P11, is essential in complex social contexts, benefiting individuals regardless of neurodiversity. 
Family members, by providing empathy, advice, and emotional support, play a vital role in improving the mental well-being of Seekers. 
Striking a balance between the family's assistance and Seeker's autonomy is another significant factor. 
Success and independence for Seekers not only benefit them but also create positive family dynamics by reducing burdens on their families.
\paragraph{}
\textbf{From Experts to Seekers: } 
Creating awareness among Seekers is more important as Experts group participant P12 remarked, \textit{``Training the employees seemed more important than employers''}.
In a context where only a small portion of companies actively support neurodivergent individuals~\cite{mydis, worko}, training becomes essential for Seekers. 
Well-trained Seekers can effectively advocate for themselves in job searches, interviews, and negotiations. 
P12 stresses the significance of using descriptive language instead of broad labels like "autism" to convey specific challenges and accommodation needs accurately. 
Experts also emphasize enhancing Seekers' soft skills, including effective communication and understanding figurative language in neurotypical contexts. As P12 rightly points out, when employers fail to provide accommodations, it's often not due to cruelty or indifference but rather a lack of understanding. Effective self-advocacy and clear communication about accommodation needs can bridge this gap in understanding. 

\paragraph{}
\textbf{From Experts to Surroundings: } 
Expert participant P13 emphasizes the crucial role of regular communication between Seekers and Surroundings groups. 
While well-meaning parents or family members often serve as advocates, it's vital to encourage independence among the Seekers. 
This communication helps break reliance and fosters self-sufficiency for the future. 
Career coaches also actively engage with families to create a comprehensive support system. 
However, there are misconceptions among family members, such as unrealistic expectations of quick and easy job placement.
P15 highlights the reality that job searching can be a lengthy process, it's essential to consider the time and effort required.
As P15 mentioned, \textit{``You could contact a hundred employers; you could wait a year before you find someone a job. It's a shame because a lot of individuals and their parents expect to get a job in a month, which doesn't happen''}.
\paragraph{}
\textbf{From Seekers to Employers: }
Job seekers with autism have clear expectations for employers to create a supportive and inclusive work environment. 
They urge employers to provide more context in job descriptions (P5, P18, P8) prioritize essential skill sets, and explicitly communicate their commitment to a neurodivergent-friendly workplace~\cite{Lashkari_2023, annabi_locke_2019}. 
Additionally, Seekers would appreciate it if employers focused on aptitude and potential rather than just skill sets. 
Changing the perception of neurotypical individuals, shaped by stereotypes, is also a priority. 
Seekers wish for tools or initiatives that can challenge and alter these assumptions (P4), promoting a more open and inclusive job market where individuals with autism can thrive based on their true potential and abilities.
\paragraph{}
\textbf{From Experts to Employers: }
One common misconception among employers is the belief that accommodating individuals with autism is financially costly. 
Experts play a vital role in dispelling such misconceptions and raising awareness about the importance of autism support in the workplace. 
Accommodations, which can include adjustments in lighting, noise control, or increased empathy, aim to create a supportive environment for employees to perform at their best. 
The absence of these accommodations often stems from a lack of understanding rather than cruelty from neurotypical perspectives. 
Experts advocate for neurodiversity training for employers and recruiters, stressing the need for an inclusive hiring process that values the unique perspectives and talents of Seekers.
As P13 mentioned, \textit{``I've been hiring individuals who are neurodivergent because I value the unique perspective they bring.''}
While some companies focus on recruiting individuals with autism, there's a need for a broader cultural change within organizations to fully support neurodiversity in the workplace, as highlighted by P14.





% they can focus on requesting specific accommodations they may need for the interview and explain how these accommodations will enable them to perform at their best.
% This can also be done by family members on their behalf, for example, P11 advocated for her son by sending an email to the employer about his special need and it was successful.


% Providing resources and materials, such as resume templates, interview questions, and career assessments is effective in preparing Seekers for their job hunt.


 



% As P1 mentioned, \textit{``I saw many people working in labs who would say something like, "I just talked to the professor and asked to work in the lab." That wasn't very helpful for me since it didn't come to me naturally''}.

% P16 also doubted his qualifications, \textit{``I think my bigger challenge is that I don't have the right degree. I don't have the right work history''}.
% Doubts when choosing a career were another concern raised by participants. 
% For P17 expressed frustration when supporting a family member: \textit{``I think the hardest thing is everything out there is set up as if you have a career that you already know what you want to do. Whether it's a doctor, a lawyer, a pipe-fitter, or an electrician, it doesn't matter. I don't know something that will be easy for him''}. 

% P5 raised an issue with the search results,\textit{``I found LinkedIn and those sorts of things exhausting. I mean It's really hard to find things on them. You search for a term, and like 80 things that are relevant come up''}.




% P16 also mentioned success with a direct referral, \textit{``I asked one of my friends if he would be a reference and he said one of the partners was his mutual friend who works for them. So I ended up contacting her, and she gave me an internal reference, so that helped''}.

% for P20: \textit{``Throughout the process, I started being more aligned with the needs and expectations that I wanted from a role and the topic I'd be working on. So I started applying to more excessively related things''}.

% For P15, \textit{``Everything's a little individualized for everyone. Some of my participants are lower-functioning, I'm going to do more for them than my higher-functioning folks''}. 
% P8 was unaware of the process for approaching someone to request a reference letter.
% as she mentioned, \textit{``Sometimes people ask for references and that was also something I hadn't received and still haven't a lot of guidance on how to approach someone to ask for a reference''}.
% Keeping track of the applications is hard, as P4 remarked, \textit{``Writing documents was fine, it was organizing, getting them submitted and getting the stuff into the right fields for the Ph.D. application process, when I was doing 10 applications at once''}. 
% Sometimes feedback received from career coaches does not match their expectations, which can undermine the confidence of the job seekers.
% P8 was assured by career support services that she had been well-prepared for job hunting; however, her real-life experience did not reflect that, \textit{``I had been told so frequently by career services that I was ready. My skills were where they needed to be, my resume was what it needed to be, and I shouldn't be having so many difficulties in the job search''}.

% Some participants felt that success in the interviews was not solely determined by their answers and experiences, but also by their behavior.
% Our participants also emphasized the usefulness of scripting as a preparation strategy for interviews.
% Therefore, anticipating the  interview questions and practicing them in advance is helpful.
% As P5 mentioned, \textit{``So I attended a social event that was for new grads, and I was glad about that too because it meant that they weren't going to be like, 'Oh, we're looking for someone with years of experience''}.
% For instance, P11 shared her experience in which a program manager provided feedback about her son, referring to the challenges related to teamwork, supporting others, and reading social cues.
% P11 advised her son to take their feedback seriously, maintain contact with the person, and demonstrate a genuine commitment to self-improvement. 
% This approach led to a success story for him.
% As P14 said, \textit{``I begin with a functional assessment. Do they live alone? How is their overall well-being outside of work? Establishing a social network and support structures often precedes job considerations. Progressing to job search, I guide them through understanding where to begin''}. 
% As P14 said, \textit{``I begin with a functional assessment. Do they live alone? How is their overall well-being outside of work? Establishing a social network and support structures often precedes job considerations. Progressing to job search, I guide them through understanding where to begin''}. 
% , \textit{``A lot of times they'll say they can do a lot more than what they're capable of, which only hurts the individual in the end. But that's why we do a lot of these assessments so we can read what is appropriate for them''}.
% As P19 said, \textit{``initial intake is very important. It allows me to introduce myself, to learn more about them. I always like to meet parents or other relatives who are involved with them as well, from a support standpoint. Because that helps as well, we want to form a job development team''}.

% Also paying attention to details, particularly in social contexts for example, where remembering a person's name is important.
% Failing to keep track of time can result in missing important events. 
% These barriers can significantly impact the attainment of an educational degree, such as a college education.
% For instance, P11 mentions, \textit{``one of his weaknesses was keeping all the balls in the air, trying to manage five classes, assignments across five classes and the time management and other issues. So, college was a struggle and we brought him home''}.


% Therefore, it is highly recommended to self-advocate and communicate regarding accommodation needs effectively so that employers can readily understand and provide the necessary support.



==> subsections/999_ray.tex <==
Ray will use this block:
designing/adopting the new socialware entails understanding the context of use thus empirical study required~\cite{ehrlich1987strategies}

challenges in designing socialware~\cite{grudin1988cscw}
challenges in designing socialware~\cite{grudin1994groupware}

groupware conflict resolve~\cite{miranda1993impact}

small group decision making~\cite{harris2018small}

coordination - managing dependencies between activities -impoact of it~\cite{malone1994interdisciplinary}

social-technical gap~\cite{ackerman2000intellectual} 
mitigating social-techical gap is the fundamental challenge in cscw...
flexible, nuanced, and contrextuali

awareness, division of labor, persistence are important. searchtogether~\cite{morris2007searchtogether}

https://pressbooks.pub/smallgroup/chapter/decision-making-in-groups/
``advantage of drawing from the experiences and perspectives of a larger number of individuals. Hence, the ideas have the potential to be more creative and lead to a more effective decision.''

group decision-making~\cite{hong2018collaborative, }
collaborative informaton-seeking~\cite{hong2019design}

structures that enable and constrain the future action based on social collaboration~\cite{scott1992microlevel}

collaborative sequencing~\cite{kim2021supporting}

infovis collaborative visual analytics~\cite{heer2007design}
